Polynomial Complexity of Inversion of sequences and Local Inversion of Maps

This Paper defines and explores solution to the problem of \emph{Inversion of a finite Sequence} over the binary field, that of finding a prefix element of the sequence which confirms with a \emph{Recurrence Relation} (RR) rule defined by a polynomial and satisfied by the sequence. The minimum number of variables (order) in a polynomial of a fixed degree defining RRs is termed as the \emph{Polynomial Complexity} of the sequence at that degree, while the minimum number of variables of such polynomials at a fixed degree which also result in a unique prefix to the sequence and maximum rank of the matrix of evaluation of its monomials, is called \emph{Polynomial Complexity of Inversion} at the chosen degree. Solutions of this problems discovers solutions to the problem of \emph{Local Inversion} of a map $F:\ftwo^n\rightarrow\ftwo^n$ at a point $y$ in $\ftwo^n$, that of solving for $x$ in $\ftwo^n$ from the equation $y=F(x)$. Local inversion of maps has important applications which provide value to this theory. In previous work it was shown that minimal order \emph{Linear Recurrence Relations} (LRR) satisfied by the sequence known as the \emph{Linear Complexity} (LC) of the sequence, gives a unique solution to the inversion when the sequence is a part of a periodic sequence. This paper explores extension of this theory for solving the inversion problem by considering \emph{Non-linear Recurrence Relations} defined by a polynomials of a fixed degree $>1$ and satisfied by the sequence. The minimal order of polynomials satisfied by a sequence is well known as non-linear complexity (defining a Feedback Shift Register of smallest order which determines the sequences by RRs) and called as \emph{Maximal Order Complexity} (MOC) of the sequence. However unlike the LC there is no unique polynomial recurrence relation at any degree.

==> deleted.tex <==
@article{Nied,
  title={Linear Complexity and Related Complexity Measures for Sequences},
  author={H. Niederreiter},
  editor={T. Johansson and S. Maitra},  
  journal={INDOCRYPT 2003, LNCS},
  volume={2904},
  number={1},
  pages={1-17},
  year={2003},
  publisher={Springer Verlag Berlin Heidelberg}
}
Harald Niederreiter
T. Johansson and S. Maitra (Eds.): INDOCRYPT 2003, LNCS 2904, pp. 1–17, 2003. ⃝c Springer-Verlag Berlin Heidelberg 2003

Entropy 2015, 17, 1936-1945; doi:10.3390/e17041936
entropy
ISSN 1099-4300
www.mdpi.com/journal/entropy
Article
On Nonlinear Complexity and Shannon’s Entropy of Finite
Length Random Sequences
Lingfeng Liu 1,
*, Suoxia Miao 2 and Bocheng Liu 1
1 School of Software, Nanchang University, Nanchang 330031, China; E-Mail: jsjjcjx@163.com
2 Faculty of Science, Nanchang Institute of Technology, Nanchang 330099, China;
E-Mail: Miaosuoxia1215@nit.edu.cn
* Author to whom correspondence should be addressed; E-Mail: vatanoilcy@163.com;
Tel.:+86-13047912526.
Academic Editor: J. A. Tenreiro Machado
Received: 25 January 2015 / Accepted: 18 March 2015 / Published: 1 April 2015


\subsubsection{Inversion of iterative sequences with quasi-periodic extension}
It is instructive to look at the case when $F$ and $y$ are such that the sequence $S(M)$ for a large enough $M$ is not periodic. Then it is quasi-periodic with a pre-period $r$ and period $N$ such that $F^{(r+k)}(y)=F^{(N+r+k)}$ for any $k\geq 0$. In such a case of $(F,y)$, inverse of $S(M)$ for $M<N$, . can be found by polynomial RRs since $F^{(r)}(y)=F^{(r+jN)}(y)=F^{(jN)}(F^{(r)}(y))$ for $j\geq 0$ hence the iterative sequence $S(F,z,M-r)$ for $z=F^{(r)}(y)$ has periodic extension. Hence PCI$(z)$ of this sequence at degree $d$, exists and the PCI of the original sequence can be considered as
\[
\mbox{PCI}=r+\mbox{PCI}(z)
\]
at any prescribed degree $d$. This shows that complexity of inversion of $S(F,y,M)$ is primarily dominated by the complexity of the cycle detection algorithm once the pre-period $r$ is computed. Hence it follows that if it is not known whether $S(F,y,M)$ extends to a periodic sequence by polynomial RRs, then the complexity of inversion by this approach of discovering RRs as rules satisfied by a sequence is dominated by cycle detection. 

Theorem \ref{ThInverse} has a converse statement which is useful for computational purpose. This converse statement is presented as 

\begin{remark}[Converse of Theorem \ref{ThInverse}]\label{ThConvInverse}
If $s_{(-1)}$ is a prefix to the sequence $S(M)$ then all polynomials $f$ in $m$ variables of degree at most $d$, whose Hankel matrices $H(S)$ and associated vectors $v_h$, $v_g$ satisfy conditions (\ref{Solvabilitycond}), (\ref{Constancycond}) define RRs for $S(M)$ and for which $s_{(-1)}$ is the unique inverse. Thus
    \[
    s_{(-1)}=s_{(m-1)}+<v_g,\bar{b}>
    \]
    The solutions of (\ref{Solvabilitycond}) and (\ref{Constancycond}) are the co-efficients of the set of all such polynomials $f$ are associated with the unique inverse.
\end{remark}

\begin{remark}\emph{Following observations clarify the conditions of the above theorem.
\begin{enumerate}
    \item Existence of a polynomial defining the RRs for $S(M)$ in the set $P(m,d)$ such that the polynomial also determines an inverse is assured by the first condition (\ref{Solvabilitycond}). This condition is also necessary for existence of a RR by a polynomial in $P(m,d)$ which determines an inverse.
    \item Once the existence condition above is satisfied, the set of all polynomials in $P(m,d)$ which determine a uniqu inverse satisfies the second condition (\ref{Constancycond}). This condition is also necessary for any subset of associated polynomials in $P(m,d)$ to determine a unique inverse of the sequence.
    \item Given that both the above conditions are satisfied by a subset of polynomials in $P(m,d)$ the unique inverse is given by the expression (\ref{TheInverse}).
    \item If two polynomials in $P(m,d)$ satisfy both conditions (\ref{Solvabilitycond}) and (\ref{Constancycond}) then they determine the same inverse. Hence they may be called equivalent. This is an equivalence relation on $P(m,d)$ and hence polynomials in $P(m,d)$ satisfying both of these conditions form a partition of the set of associated polynomials of $S(M)$ such that each equivalence class corresponds to a unique inverse. Hence the set of associated polynomials in $P(m,d)$ determine a unique inverse iff they form a single equivalence class. 
    \item The equivalence class of polynomials $f$ in $P(m,d)$ which determine the unique inverse of $S(M)$ is described in terms of vectors $v_h(S)$ and $v_g(S)$ of the components $h$ and $g$ of $f$ evaluated at first $m$ terms of $S$. Let $\bar{a}$ and $\bar{b}$ denote the coefficients of $h$ and $g$ respectively. Then $h$ satisfies $<v_h(S),\bar{a}>=1$ while $g$ satisfies $<v_g(S),\bar{b}>$ is constant for all coefficients in the equivalence class. Since we are working with the binary field, the constant is either $0$ or $1$. Hence if $P(m,d)$ is partitioned in two subsets one for which $<v_g(S),\bar{b}>=0$ and another for which $<v_g(S),\bar{b}>=1$ then there is no unique inverse for $S(M)$ by a RR defined by a polynomial in $P(m,d)$. Hence for existence of a unique inverse we must have the value of $<v_g(S),\bar{b}>$ to be exactly either $0$ or $1$ for all associated polynomials $f$.
\end{enumerate}
}
\end{remark}

\begin{definition}\label{PCofuniqueI}
The \emph{Polynomial Complexity of Unique Inversion of $S(M)$ at degree $d$} of a given scalar sequence $S(M)$, is the smallest number $m$ of variables for which there exists $1\leq d\leq m$ such that all polynomials $f$ in $P(m,d)$ which defines a RR for $S(M)$ determine a unique inverse $s_{(-1)}$. We denote this complexity $m$ as $\PCUId$ of $S(M)$. If $S(M)$ is a vector sequence then, the smallest $m$ for which there exists $1\leq d\leq m$ such that all polynomial $f$ in $P(m,d)$ which satisfy RRs for all co-ordinate sequences $S(i)$ determine unique inverses $s_{(-1)}(i)$ for each $S(i)$, (thereby determine a unique vector $S_{(-1)}$ as inverse) is called the Polynomial Complexity of Unique Inversion at degree $d$ denoted \PCUId, of $S(M)$.
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%% Algorithms
\subsubsection{Procedure for Inversion of a scalar sequence}
First consider a scalar sequence $S(M)$ and fix a degree $d$. The procedure $\mbox{I\textsc{nversion}}()$ described in Algorithm \ref{Inverse} returns a Boolean output $\mbox{\rm Invertible}= T/F$. If it is $T$, returns $(m, d,\bar{a},\bar{b}, s_{(-1)})$ where $m$ is the PCI at degree $d$ and for one $f$ associatd with RRs solution $\bar{a}$, $\bar{b}$ of co-efficients of polynomials $h$, $g$ and $s_{(-1)}$.

\begin{algorithm}\label{Inverse}
\caption{Algorithm computes PCI at degree $d$ of a scalar sequence or returns Invertible$=False$}
\begin{algorithmic}[1]
\Procedure{Inversion()}{at degree $d$}
\State \textbf{Input} Scalar sequence $S(M)$, degree $d$.
\State \textbf{Output} $(\mbox{Boolean:Invertible}=T/F)\mbox{OR}(m,\bar{a},\bar{b},s_{(-1)})$.
\State \%$m=$PCI at degree $d$, $\bar{a}$, $\bar{b}$ co-efficients of $h$, $g$, $s_{(-1)}$ the Inverse\%
\State $m=1$, Define $f$, $h$, $g$ with co-efficients $\bar{a}$, $\bar{b}$. 
\Repeat
\State Compute Hankel matrix $H(S)$ of $f$, matrix $H_{22}$, vectors $\bar{s}_2$, $v_h$, $v_g$.
\State Boolean:Flag$:=\mbox{\rm False}$ (\%for satisfying conditions of Theorem 1.)\%
\State Compute Boolean $t_1=(\rank H_{22}(S)=\rank [H_{22}(S),\bar{s}_2])$. 
\State Compute Boolean $t_2=(\rank H_{22}(S)=\rank\barr{l}H_{22}(S)\\v_g\earr)$.
\State Compute Boolean Flag$=t_1\mbox{ AND }t_2$
\If {Flag$=\mbox{\rm True}$} 
\State Compute one solution $\bar{a}$, $\bar{b}$ of (\ref{ReducedeqnbyE})
\State Return Invertible$=\mbox{\rm True}$, $(m,\bar{a},\bar{b})$, $\mbox{\rm Inverse}=s_{(-1)}$
\Else {\ $m\leftarrow m+1$}
\EndIf
\Until {m=M}
\State Return Invertible$=\mbox{\rm False}$ \%Inverse does not exist\%
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsubsection{Procedure for verifying a polynomial generating a RR}
Previous procedure I\textsc{nversion} computes the \PCUId\ at degree $d$ for a scalar sequence. Following procedure V\textsc{erify}, verifies whether a given polynomial $f$ satisfies the RRs of a given scalar sequence and existence of an inverse. This is described by Algorithm \ref{Verify}.

\begin{algorithm}\label{Verify}
\caption{Algorithm to verify whether a given function $f$ satisfies a RR for a scalar sequence $S(M)$}
\begin{algorithmic}[1]
\Procedure{Verify()}{\% Given $f$\%}
\State \textbf{Input} Scalar sequence $S(M)$, $m$, co-efficients of $f$: $\bar{a}$, $\bar{b}$.
\State \textbf{Output} Boolean $V=\mbox{\rm T/F}$.
\State Compute $H(S)$ for $f$, $v_h$, $v_g$, $H_{22}(S)$, $\bar{s}_2$.
\State Compute Boolean $t_1=(\rank H_{22}(S)=\rank [H_22(S),\bar{s}_2]$.
\State Compute Boolean $t_2=(\rank H_{22}(S)=\rank\barr{l}H_{22}(S)\\v_g\earr)$.
\State Compute $V=t_1\mbox{\rm AND }t_2$.
\State Return $V$.
\EndProcedure
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%
